The LOFAR Two-metre Sky Survey IV. First Data Release: Photometric redshifts and rest-frame magnitudes

The LOFAR Two-metre Sky Survey (LoTSS) is a sensitive, high-resolution 120-168 MHz survey of the Northern sky. The LoTSS First Data Release (DR1) presents 424 square degrees of radio continuum observations over the HETDEX Spring Field (10h45m00s $<$ right ascension $<$ 15h30m00s and 45$^\circ$00$'$00$'$ $<$ declination $<$ 57$^\circ$00$'$00$''$) with a median sensitivity of 71$\mu$Jy/beam and a resolution of 6$''$. In this paper we present photometric redshifts (photo-$z$) for 94.4% of optical sources over this region that are detected in the Panoramic Survey Telescope and Rapid Response System (Pan-STARRS) 3$\pi$ steradian survey. Combining the Pan-STARRS optical data with mid-infrared photometry from the Wide-field Infrared Survey Explorer, we estimate photo-$z$s using a novel hybrid photometric redshift methodology optimised to produce the best possible performance for the diverse sample of radio continuum selected sources. For the radio-continuum detected population, we find an overall scatter in the photo-$z$ of 3.9% and an outlier fraction ($\left | z_{\rm{phot}} - z_{\rm{spec}} \right | / (1+z_{\rm{spec}}) > 0.15$) of 7.9%. We also find that, at a given redshift, there is no strong trend in photo-$z$ quality as a function of radio luminosity. However there are strong trends as a function of redshift for a given radio luminosity, a result of selection effects in the spectroscopic sample and/or intrinsic evolution within the radio source population. Additionally, for the sample of sources in the LoTSS First Data Release with optical counterparts, we present rest-frame optical and mid-infrared magnitudes based on template fits to the consensus photometric (or spectroscopic when available) redshift.

==> all_specz_stats.tex <==
\begin{table}
\begin{tabular}{cccc}
Subset & N & $\sigma_{	extup{NMAD}}$ & $	extup{OLF}$ \\
All & 314625 & 0.041 & 0.104 \\
Galaxies & 233002 & 0.031 & 0.034 \\
All AGN & 81623 & 0.123 & 0.306 \\
QSOs & 69251 & 0.110 & 0.274 \\
X-ray AGN & 1689 & 0.070 & 0.132 \\
IR AGN & 34527 & 0.083 & 0.169 \\
\end{tabular}
\end{table}


==> radio_specz_stats.tex <==
\begin{table}
\begin{tabular}{cccc}
Subset & N & $\sigma_{	extup{NMAD}}$ & $	extup{OLF}$ \\
All & 27821 & 0.038 & 0.066 \\
Galaxies & 20506 & 0.031 & 0.013 \\
All AGN & 7315 & 0.087 & 0.215 \\
QSOs & 6299 & 0.081 & 0.198 \\
X-ray AGN & 400 & 0.056 & 0.125 \\
IR AGN & 4838 & 0.086 & 0.193 \\
\end{tabular}
\end{table}

